Partitioning through projections: strong SDP bounds for large graph partition problems

The graph partition problem (GPP) aims at clustering the vertex set of a graph into a fixed number of disjoint subsets of given sizes such that the sum of weights of edges joining different sets is minimized. This paper investigates the quality of doubly nonnegative (DNN) relaxations, i.e., relaxations having matrix variables that are both positive semidefinite and nonnegative, strengthened by additional polyhedral cuts for two variations of the GPP: the $k$-equipartition and the graph bisection problem. After reducing the size of the relaxations by facial reduction, we solve them by a cutting-plane algorithm that combines an augmented Lagrangian method with Dykstra's projection algorithm. Since many components of our algorithm are general, the algorithm is suitable for solving various DNN relaxations with a large number of cutting planes. We are the first to show the power of DNN relaxations with additional cutting planes for the GPP on large benchmark instances up to 1,024 vertices. Computational results show impressive improvements in strengthened DNN bounds.

==> Hager_datafile1.tex <==
n,k,UB,DNN_lb,round_DNN_lb,DNN_cputime,DNN_clocktime,cuts_lb,round_cuts_lb,cuts_cputime,cuts_clocktime,imp_lb,imp_lb_round,TotalTriCuts,TotalCliqueCuts,numClustTri,numClustCliq,cut_add_occasions_total,iter,stopflag,sigma,graph,graph_string,
124,2,13,7.28532052225482,8,9,1.2521323,12.0128311074534,13,160.84375,31.5573908,0.648909072807054,0.625,3298,1166,41,18,12,848,1,0.018322034333498,G124.02,\(G_{124,2.5}\),
124,2,63,46.7102970636413,47,4.703125,0.6530695,61.338334386335,62,341.140625,72.2986922,0.313165152916143,0.319148936170213,4354,482,41,9,13,1325,2,0.011571402817698,G124.04,\(G_{124,5}\),
124,2,178,152.857252115462,153,2.84375,0.4007673,170.877609333514,171,48.921875,9.8563522,0.11789010314303,0.117647058823529,2663,432,19,6,9,570,2,0.015559870167661,G124.08,\(G_{124,10}\),  
124,2,449,418.672727417812,419,2.6875,0.3876029,439.95858648967,440,34.0625,6.6688111,0.050841284081578,0.050119331742244,2266,509,13,7,8,485,2,0.011687184131925,G124.16,\(G_{124,20}\),
250,2,29,15.1588063084243,16,35.171875,4.8282195,28.3040857716572,29,4019.859375,968.0517114,0.867171147633676,0.8125,15865,2135,87,23,24,2068,1,0.005257466832045,G250.01, \(G_{250,2.5}\),
250,2,114,81.5222883170643,82,18.921875,2.6655993,104.999755400908,105,874.734375,174.1071799,0.28798832280729,0.280487804878049,10063,374,92,5,14,1184,2,0.008698751175913,G250.02,\(G_{250,5}\),  
250,2,357,303.016218855567,304,15.09375,2.102401,330.402579084339,331,164.03125,27.7361504,0.090379189378724,0.088815789473684,5352,415,42,5,9,575,2,0.011940455580504,G250.04,\(G_{250,10}\),  
250,2,828,746.265550639492,747,12.734375,1.7741714,780.743686114921,781,54.390625,10.594845,0.046200893831806,0.045515394912985,4516,617,13,5,7,484,2,0.010102480305792,G250.08,\(G_{250,20}\),
70,2,7,2.91000531699043,3,1.25,0.1934524,6.01817711868984,7,6.921875,2.4224597,1.06809832392813,1.33333333333333,474,366,25,9,4,351,1,0.037905525988941,mesh.70.120 ,mesh.70.120 ,
74,2,8,3.55540264499326,4,1.453125,0.1955245,7.14849283239675,8,10.53125,3.7442161,1.01060007717081,1,575,313,20,12,4,518,1,0.024743678047277,mesh.74.129 ,mesh.74.129,
138,2,8,1.54350478454276,2,10.25,1.4192829,7.10614672053748,8,618.53125,124.3833485,3.60390326722736,3,5298,3810,29,19,22,1135,1,0.017955827117338,mesh.138.232 ,mesh.138.232,
148,2,7,2.68620603060218,3,16.0625,2.250933,6.15932747322803,7,36.0625,6.1472518,1.29294678183984,1.33333333333333,1064,1156,27,16,5,481,1,0.019345394243569,mesh.148.265 ,mesh.148.265,
274,2,7,1.14442361066238,2,96.796875,13.6903877,6.09040916433291,7,3815.75,1000.6020062,4.32181362529549,2.5,14038,7334,38,33,26,1926,1,0.005738000467411,mesh.274.469 ,mesh.274.469,
82,2,13,4.88131927305449,5,1.46875,0.2155911,12.4266512501266,13,20.4375,6.2271306,1.54575670121053,1.6,515,715,19,16,5,357,1,0.019983245569072,KKT_lowt01,KKT.lowt01,

==> Hager_datafile2.tex <==
n,k,UB,DNN_lb,round_DNN_lb,DNN_cputime,DNN_clocktime,cuts_lb,round_cuts_lb,cuts_cputime,cuts_clocktime,imp_lb,imp_lb_round,TotalTriCuts,TotalCliqueCuts,numClustTri,numClustCliq,cut_add_occasions_total,iter,stopflag,sigma,graph,graph_string,
45,3,1408,1260.925072706,1261,2.4375,0.0395015,1407.65226165996,1408,82.328125,60.7316745,0.116364716770265,0.116574147501983,372,438,13,48,6,1426,1,0.0240627545932,cb.45.98,cb.45.98,
69,3,10,3.60774014739462,4,1.203125,0.0418025,8.59740316941194,9,1631.703125,1093.3881143,1.38304390509407,1.25,1375,4421,21,109,28,1266,2,0.023513454141646,Mesh.69.212,mesh.69.212,
138,3,13,1.48106029608232,2,1.9375,0.2962077,11.353413702298,12,3642.34375,1019.3264416,6.665733618226,5,3862,8558,28,108,30,1877,4,0.012796939168501,mesh.138.232 ,mesh.138.232,
124,4,23,12.755552970779,13,1.203125,0.181248,20.2527124193492,21,974.875,215.180769,0.587756521865029,0.615384615384615,5124,456,53,14,15,1741,2,0.010713864398436,G124.02, \(G_{124,2.5}\),
124,4,104,79.1993802471889,80,0.65625,0.0919775,93.600885306963,94,251.8125,53.8556599,0.181838608014679,0.175,3160,188,64,7,9,1003,2,0.010065393087738,G124.04, \(G_{124,5}\),  
124,4,290,250.082497435608,251,0.609375,0.0851899,260.760270175558,261,25.90625,5.5379865,0.04269700138731,0.039840637450199,1519,130,21,6,6,325,2,0.013978696815355,G124.08, \(G_{124,10}\),  
124,4,720,659.717087146369,660,0.40625,0.0659026,669.297658240917,670,11.96875,3.0386311,0.014522241853685,0.015151515151515,949,221,15,7,4,234,2,0.012121793719145,G124.16, \(G_{124,20}\),  
128,4,30,14.896245442461,15,1.984375,0.2703313,26.3925422893492,27,1064.984375,235.3620665,0.771758017232892,0.8,4974,402,32,11,14,2047,2,0.007349175551335,se7,se7,
148,4,22,8.13242024394805,9,1.453125,0.2041026,21.2315806588939,22,2309.265625,101.94,1.61073333915496,1.44444444444444,3382,458,51,12,10,1197,2,0.009396227830062,mesh.148.265,mesh.148.265,
70,5,20,11.2084123567966,12,0.1875,0.0365033,17.6307221964897,18,126.609375,97.035168,0.572990146619536,0.5,1401,279,26,16,8,1570,2,0.01992801972218,mesh.70.120 ,mesh.70.120,
115,5,104,81.7640562910578,82,4.34375,0.6181537,100.066804263274,101,989.25,208.2342546,0.223848336328415,0.231707317073171,2255,310,16,19,19,2193,2,0.007790624415977,KKT_putt01,KKT.putt01,
250,5,58,26.2292122746384,27,4.640625,0.6659508,49.2069810577526,50,3771.796875,839.0372587,0.87603731833502,0.851851851851852,12682,68,58,12,17,2047,2,0.005143941462304,G250.01, \(G_{250,2.5}\),
250,5,209,146.808076998499,147,2.78125,0.3737951,171.630538986793,172,525.859375,97.9800455,0.16908103760904,0.170068027210884,6747,3,111,1,9,726,2,0.006928743184008,G250.02, \(G_{250,5}\),  
250,5,629,522.301143965622,523,2,0.2791562,539.671115787788,540,55.609375,11.7411799,0.033256622205119,0.032504780114723,2605,5,33,2,5,257,3,0.00969323518559,G250.04, \(G_{250,10}\),  
250,5,1418,1262.60665615399,1263,1.953125,0.2524076,1276.16963629761,1277,17.984375,4.8958988,0.010742047079757,0.011084718923199,1545,8,12,1,3,176,3,0.008315929654591,G250.08, \(G_{250,25}\),  
138,6,24,8.20108672001771,9,0.734375,0.1186149,20.6493432385146,21,1618.59375,332.9038984,1.51787890354975,1.33333333333333,5974,650,31,16,16,1605,2,0.012560300273065,mesh.138.232,mesh.138.232,

==> Hager_datafile3.tex <==
n,k,UB,DNN_lb,round_DNN_lb,DNN_cputime,DNN_clocktime,cuts_lb,round_cuts_lb,cuts_cputime,cuts_clocktime,imp_lb,imp_lb_round,TotalTriCuts,TotalCliqueCuts,numClustTri,numClustCliq,cut_add_occasions_total,iter,stopflag,sigma,graph
20,2,6,2.67284608409418,3,0.125,0.1311543,5.9292229914497,6,1.171875,1.0921636,1.21831815409569,1.24479817064864,23,97,8,8,2,367,1,0.085988718406895,10x2g
30,2,19,11.0337154881111,12,0.375,0.0390259,18.2553026384787,19,8.90625,4.3352751,0.654501845561353,0.721994736992505,281,169,26,8,5,581,1,0.051117224634652,5x6g
32,2,8,2.95150392107908,3,0.84375,0.1048865,7.59506911103735,8,4.9375,1.9107654,1.5732878268583,1.71048259257442,193,191,12,10,4,341,1,0.077126377265991,2x16g
36,2,6,2.40619220696752,3,1.46875,0.1864142,5.27092404061025,6,3.09375,1.3509799,1.19056649977813,1.49356638369372,146,178,18,8,3,251,1,0.063159633389723,18x2g
38,2,6,1.3604409271326,2,1.21875,0.1583066,3.22256614238834,4,69.578125,29.4518185,1.36876594794935,1.94022321750552,692,993,24,18,16,1184,2,0.04359250428961,2x19g
40,2,18,11.2749463903653,12,0.625,0.0872578,17.1379356341833,18,1.796875,0.8046491,0.520001518484208,0.596459918903154,91,149,10,14,2,254,1,0.053792153496746,5x8g
42,2,10,3.60034402168058,4,0.875,0.1105669,9.16690935685816,10,13.296875,6.5553865,1.54612039895543,1.77751235431446,443,439,36,18,7,511,1,0.049680646363694,3x14g
50,2,22,11.156841404806,12,1.625,0.2046318,21.4999081263198,22,7.421875,3.3131126,0.927060477623922,0.971884263813513,460,290,21,13,5,479,1,0.041482727643,5x10g
60,2,28,13.4511158533319,14,0.84375,0.1517521,27.0525727567161,28,51.8125,17.602385,1.0111768459726,1.08161168971452,1117,1223,33,21,13,696,1,0.027105189093022,6x10g
70,2,23,10.912006976557,11,1.84375,0.2663967,22.3604446008209,23,52.8125,16.9632565,1.04915966868967,1.10776991340021,1081,1229,27,17,11,792,1,0.031402956224273,7x10g
20,2,28,24.4538929113356,25,0,0.0094051,27.0187856319213,28,0.203125,0.1457136,0.104886887739528,0.145011966050632,44,16,7,3,1,135,1,0.103623224684692,4x5t
24,2,9,4.42087143426146,5,0.109375,0.1121888,8.72848177957561,9,1.65625,1.3354971,0.97438037033388,1.03579772310287,134,82,8,6,3,373,1,0.102373846896697,12x2t
30,2,31,22.647197566313,23,0.25,0.023198,30.6803681615845,31,2.8125,1.0318173,0.354709255825126,0.368822783005679,93,87,19,8,2,202,1,0.056357650360659,6x5t
40,2,33,20.2710136041984,21,0.359375,0.0511059,32.0606774959231,33,3.296875,1.8134599,0.581602090646464,0.62794030157255,348,132,13,8,4,277,1,0.059385502105219,8x5t
46,2,9,1.97739334452204,2,2.421875,0.3130555,6.16254068175961,7,64.984375,17.0004204,2.11649712933021,2.54001393773882,1094,1083,35,16,18,634,3,0.050893298180796,23x2t
48,2,24,10.9881549864818,11,1.359375,0.1822733,23.6632275301234,24,11.125,4.4086229,1.15352145644425,1.18417013861982,539,325,17,12,6,446,1,0.040243355424343,4x12t
50,2,33,16.5228931915164,17,0.625,0.0915555,32.351670778018,33,6.890625,3.8967932,0.957990674092647,0.997228912485114,513,237,15,13,5,348,1,0.040136938947935,5x10t
60,2,43,19.465582601454,20,0.53125,0.0835619,41.9970871828879,42,176.171875,126.5141345,1.15750476329185,1.15765440264104,1412,928,27,22,13,1537,2,0.018280015389665,10x6t
70,2,45,20.3035959247191,21,0.5625,0.0990192,44.2191455781885,45,22.421875,8.1274417,1.17789724254475,1.21635616502856,1120,350,24,14,7,505,1,0.029199655573273,7x10t
80,2,43,23.453124690994,24,0.921875,0.1482302,42.9916163467829,43,210.46875,62.0063968,0.833086930343729,0.833444394576216,2263,2150,43,31,19,890,1,0.019493728915133,10x8t
20,2,118,111.951416329426,112,0.03125,0.0052936,117.882216849025,118,0.140625,0.1383075,0.05297655638538,0.054028648041179,44,16,4,2,1,139,1,0.046102988978044,2x10m
30,2,270,258.142277957366,259,0.25,0.0326936,269.72473894688,270,1.53125,0.5973748,0.044868516235171,0.045934831506339,144,36,16,3,2,219,1,0.031485122843803,6x5m
34,2,316,296.148636436583,297,0.125,0.0280952,312.180479488128,313,28.90625,18.7615395,0.054134448310986,0.05690170910858,432,486,16,14,9,1203,2,0.023986073591854,2x17m
40,2,436,423.770216212679,424,0.125,0.0238187,435.137674282675,436,2.0625,0.9097578,0.026824580008452,0.028859469871718,156,84,9,6,2,200,1,0.022893632115746,10x4m
50,2,670,653.963565846674,654,0.375,0.0507522,669.999579557542,670,5.140625,1.9024189,0.024521264713129,0.024521907627322,346,104,28,6,3,258,1,0.013914863545566,5x10m
52,2,721,694.46112607877,695,0.375,0.0510391,720.542576108751,721,6.890625,4.4051324,0.037556385880443,0.038215060461455,459,477,18,16,6,349,1,0.013709740558404,4x13m
52,2,721,694.46112607877,695,0.3125,0.0510203,720.465661913168,721,8.1875,4.6662872,0.037445632099281,0.038215060461455,440,496,14,16,6,398,1,0.015157280975915,13x4m
54,2,792,761.808404846158,762,0.453125,0.068726,791.32275654331,792,4.390625,2.1326703,0.038742486312044,0.03963148077887,410,238,17,9,4,299,1,0.014405041462556,9x6m
60,2,954,931.768614444553,932,0.640625,0.0978824,953.999530543089,954,3.8125,1.6839438,0.023858837649075,0.023859341483293,460,80,10,4,3,330,1,0.010191728286828,10x6m
70,2,1288,1258.2582145509,1259,0.984375,0.1393563,1287.85225560726,1288,10.640625,3.364636,0.023519847288995,0.02363726706105,624,216,40,7,4,372,1,0.01026426811802,10x7m
20,2,401,392.008780021161,393,0.015625,0.0152589,400.723190231697,401,0.515625,0.4987321,0.022230140381207,0.022936271933383,80,40,8,5,2,164,1,0.030176787882504,v000
20,2,21,18.322201605002,19,0.015625,0.0199022,20.7002222923156,21,0.765625,0.7396305,0.129789025280914,0.146150471036568,57,63,14,9,2,190,1,0.083808060712381,v090
30,2,900,877.921003322586,878,0.125,0.0259051,899.326862272091,900,3.34375,1.6734806,0.024382443145217,0.025149183803388,284,166,10,8,5,289,1,0.022118575086574,t000
30,2,397,370.048476968143,371,0.375,0.0575638,396.38483568396,397,6.3125,3.4901874,0.071170023267206,0.072832411722579,343,197,14,7,6,449,1,0.025881875330817,t050
30,2,24,20.7049407079921,21,0.5,0.0611332,23.2507514766938,24,0.9375,0.3608227,0.122956679983103,0.159143623663506,65,25,16,7,1,154,1,0.060177572513007,t090
40,2,1606,1577.62891134949,1578,0.25,0.032122,1605.35263473613,1606,2.515625,0.9238068,0.017573032027491,0.017983372671741,329,151,9,7,4,247,1,0.012364094469135,q000
40,2,1425,1386.49734296736,1387,0.125,0.0276375,1423.45002807775,1424,9.703125,4.4008749,0.026651825405813,0.027048488208695,404,196,10,7,5,812,2,0.013793966001942,q010
40,2,1238,1202.41873154927,1203,0.125,0.0238153,1237.55363916628,1238,8.421875,4.2541252,0.029220193178245,0.02959141230683,487,233,11,7,6,657,1,0.014362358281109,q020
40,2,1056,1015.96166328898,1016,0.125,0.0286181,1054.15837978474,1055,5.5,2.8267443,0.037596612033672,0.038425009645188,491,229,10,9,6,421,2,0.017475673275349,q030
40,2,199,168.600724647361,169,0.25,0.0356406,198.397247162767,199,9.15625,5.3148878,0.176728318206979,0.18030334932558,521,319,14,9,7,542,1,0.023530482484515,q080
40,2,63,50.6596396093662,51,0.75,0.1018958,62.3026394099793,63,3.8125,1.7929286,0.229827923972449,0.243593529006319,315,165,16,12,4,369,1,0.044079714141856,q090
50,2,1658,1592.51770272699,1593,0.375,0.0462944,1654.07744822054,1655,10.65625,4.8776922,0.038655611418408,0.039234915358251,725,325,13,8,7,529,2,0.012449063590604,c030
50,2,603,555.597247250563,556,0.5,0.0629193,599.287350054157,600,17.984375,7.1066283,0.078636283782541,0.07991895742675,817,315,15,8,9,694,2,0.018039302055415,c070
50,2,368,327.842568747166,328,0.4375,0.0847229,366.560218934566,367,38.71875,22.4801056,0.118098300459753,0.119439740246278,967,353,22,8,9,1124,2,0.0126353756493,c080
50,2,122,101.92751533877,102,0.625,0.0822683,121.013803411125,122,4.609375,1.4513728,0.187253540017326,0.196929009743016,421,179,14,7,4,348,1,0.033554898904334,c090
52,2,123,96.4090441842344,97,0.375,0.0575233,122.030492089961,123,7.84375,2.7065141,0.265757721410088,0.275813913941011,543,237,18,16,5,381,1,0.027223488872713,c290
54,2,160,134.979252197953,135,0.484375,0.071639,159.074347792995,160,6.734375,2.2761716,0.178509624276963,0.185367361239733,577,233,16,8,5,371,1,0.028716261435144,c490
56,2,177,149.244940172924,150,0.609375,0.10597,176.335299595836,177,7.953125,2.7943056,0.181516099584505,0.185969854622323,623,217,16,11,5,415,1,0.020341047856054,c690
58,2,227,185.338431627877,186,0.828125,0.1313311,222.963538698376,223,29.640625,13.6947466,0.203007583154922,0.203204311385024,1219,347,34,8,9,861,2,0.020903552417171,c890
60,2,238,200.546601592166,201,0.546875,0.0867663,237.318602269457,238,15.65625,5.9759416,0.183358882101981,0.186756584806157,886,374,19,10,7,539,1,0.017661521572038,s090
8,2,4,3.82235974827321,4,0,0.0035759,3.81050029456092,4,0.015625,0.0042158,0.003102652417174,0.046473975090137,0,0,0,0,0,69,1,0.169996442566161,db3
32,2,10,6.88423214944217,7,0.25,0.0177057,9.2578448987146,10,3.234375,1.4052376,0.344789759808545,0.452594825816602,194,94,9,6,3,349,1,0.062540758515761,db5
64,2,18,10.2250661365467,11,0.609375,0.1047288,17.0209214106277,18,15.5625,5.523415,0.664627023759883,0.760379811692751,1020,324,16,7,7,518,1,0.027969793510574,db6
128,2,30,15.1395595458436,16,2.9375,0.3963775,29.9993245456659,30,36.31,149.44,0.981518977142362,0.98156359233292,3650,958,41,11,12,910,2,0.005257474511962,db7
32,2,6,3.67623676967517,4,0.21875,0.0424353,5.13928765832103,6,1.484375,0.510789,0.397975152393444,0.632103799595627,138,54,10,5,2,163,1,0.072572693264283,m4
54,2,2,0.742544987556784,1,0.859375,0.1086551,1.1910397586013,2,0.765625,0.2616575,0.603996765933618,1.69343949998323,132,30,10,4,1,181,1,0.049143299817487,ma
60,2,3,1.20114793811338,2,0.90625,0.1429149,2.01141935848888,3,0.84375,0.4010052,0.674580869404128,1.49761074785845,90,90,7,6,1,171,1,0.044423837485729,me
70,2,7,2.91000531699042,3,1.203125,0.18982,6.02177500742118,7,6.03125,2.3871086,1.06933470954926,1.40549388660208,475,365,25,9,4,351,1,0.037892476255351,m6
74,2,4,1.09640761042306,2,1.5625,0.227905,3.09706618050823,4,14.671875,5.1721484,1.82473976928452,2.64827821512162,626,706,15,17,6,446,1,0.033448988142347,mb
74,2,6,2.27539468805532,3,1.09375,0.1612585,5.12884210916483,6,5.328125,2.2162087,1.25404503934578,1.63690516265024,420,468,15,15,4,342,1,0.036898064247179,mc
80,2,4,1.10068499029115,2,1.625,0.2423111,3.0727039563779,4,14.6875,4.7930092,1.79162883429992,2.63410061487432,567,873,12,12,6,448,1,0.035348933165545,md
90,2,4,1.03304309285502,2,1.96875,0.3079641,3.08158800251849,4,15.078125,5.1463764,1.98301980220584,2.87205531663273,915,705,14,12,6,437,1,0.031403190841836,mf
100,2,4,0.886285566199276,1,5.203125,0.7774793,3.03748458253596,4,216.75,47.3883813,2.42720754842238,3.51321803327284,2461,2639,32,22,17,922,1,0.018730182702582,m1
148,2,9,2.6862060306022,3,16.59375,2.3271692,6.98909493653794,7,283.375,49.8457697,1.60184619381973,1.60590584648145,2639,3146,41,22,14,864,3,0.010834330218625,m8
32,2,6,3.05233404130947,4,0.125,0.0215716,5.12299385807708,6,4.359375,1.8385747,0.678385716878905,0.965708837498652,248,136,18,8,4,365,1,0.063212204611372,se5
64,2,9,4.71711068572707,5,0.953125,0.1424689,8.27652429691017,9,10.546875,4.8270481,0.754574960887201,0.907947597505397,688,464,13,10,6,539,1,0.039387587733945,se6
128,2,16,7.17773505630431,8,3.921875,0.5813273,15.0231258213131,16,122.640625,25.8324598,1.09301760283254,1.2291154346728,3626,598,23,10,11,857,1,0.016047344297096,se7

==> hagerBisection_datafile1.tex <==
n,m1,UB,DNN_lb,round_DNN_lb,DNN_cputime,DNN_clocktime,cuts_lb,round_cuts_lb,cuts_cputime,cuts_clocktime,imp_lb,imp_lb_round,TotalBQPTriCuts,numClustBQPTri,cut_add_occasions_total,iter,stopflag,graph,graph_string,
124,75,12,6.00642816304654,7,77.515625,11.2857066,9.99644990405172,10,32349.90625,7077.1141511,0.664291927364263,0.428571428571429,7399,145,21,29486,3,G124.02,\(G_{124,2.5}\),
124,87,49,41.2371079908197,42,97.3125,14.2263061,48.0661872016825,49,3741.984375,616.3535168,0.165605192594569,0.166666666666667,4054,90,13,15861,1,G124.04,\(G_{124,5}\),
124,81,159,140.609002763814,141,83.609375,12.2619936,149.956147199745,150,935.734375,154.1276256,0.066476144857042,0.063829787234043,2429,46,8,12633,3,G124.08,\(G_{124,10}\),
124,75,414,398.248633598769,399,87.796875,12.9318929,411.211761499398,412,2268.96875,373.6047025,0.032550338675335,0.032581453634085,2716,44,8,19067,2,G124.16,\(G_{124,20}\),
250,175,20,11.3882646396351,12,1382.921875,202.6349095,15.6684808984494,16,26338.515625,7200.5195386,0.375844467463256,0.333333333333333,15750,170,21,38639,2,G250.01,\(G_{250,2.5}\),
250,163,101,73.3205562828957,74,887.140625,129.1125872,89.3366023109624,90,8040.28125,1710.966304,0.218438686775253,0.216216216216216,9702,90,15,23906,2,G250.02,\(G_{250,5}\),
250,150,343,288.330175081409,289,560.078125,81.5147244,309.60193682261,310,2529.9375,441.6484811,0.073775704312584,0.072664359861592,5454,57,9,16145,3,G250.04,\(G_{250,10}\),
250,175,673,626.881446757844,627,648.375,94.4700855,640.737330431435,641,2821.40625,473.6166743,0.022102877258933,0.022328548644338,4416,50,6,17655,2,G250.08,\(G_{250,20}\),
138,90,6,1.4025974834764,2,146.6875,21.5133146,5.10612560009927,6,13521.75,2647.7289652,2.64047822718425,2,7452,138,17,24424,1,mesh.138.232,mesh.138.232,
148,89,9,3.16952953947826,4,248.734375,36.9647048,7.19596938332492,8,14423.40625,3074.6816306,1.270358832027,1,7104,151,16,31656,3,mesh.148.265,mesh.148.265,
274,192,10,1.43059505963921,2,1752.203125,259.5492886,4.81725003859408,5,26217.5625,7200.5225075,2.36730509876706,1.5,15618,184,19,43682,5,mesh.274.469,mesh.274.469,
70,46,6,3.01047001318663,4,28.953125,4.5362411,5.03572934069033,6,1620.703125,374.2029683,0.672738581893375,0.5,1470,59,6,12431,1,mesh.70.120,mesh.70.120,
74,45,7,4.1092711648911,5,26.3125,4.0171084,6.11423610566219,7,139.34375,28.0147167,0.487912542229182,0.4,1110,48,4,7695,1,mesh.74.129,mesh.74.129,
82,58,13,9.31634941774573,10,23.1875,3.5715143,12.1924663910204,13,2016.625,371.4944873,0.308717164235628,0.3,984,56,3,12164,1,KKT_lowt01,KKT\_lowt01,

==> largeGraphSparse3n_datafile1.tex <==
n,k,UB,DNN_lb,round_DNN_lb,DNN_cputime,DNN_clocktime,cuts_lb,round_cuts_lb,cuts_cputime,cuts_clocktime,imp_lb,imp_lb_round,TotalTriCuts,TotalCliqueCuts,numClustTri,numClustCliq,cut_add_occasions_total,iter,stopflag,sigma,graph,graph_string,
500,2,49,24.8999946365116,25,266.625,45.8307645,40.8254010692756,41,4089.671875,1094.0907784,0.639574693297809,0.64,14593,407,73,59,10,1560,4,0.018891198031821,G500.005,\(G_{500,2.5}\),
500,2,218,155.578188913135,156,133.03125,22.596964,195.655814023588,196,904.40625,222.6049035,0.257604394230542,0.256410256410256,14597,403,38,7,10,1116,4,0.012867692662404,G500.01, \(G_{500,5}\),  
500,2,626,512.133506337669,513,94.234375,15.9009213,553.547033930157,554,413.796875,91.7493828,0.080864710236675,0.079922027290448,10989,464,47,4,9,743,2,0.016219556710487,G500.02, \(G_{500,10}\),  
500,2,1744,1565.591086041,1566,86.75,14.7806008,1612.85929173751,1613,161.90625,35.0262408,0.030191923113231,0.030012771392082,8075,743,18,5,7,547,3,0.013176409604152,G500.04, \(G_{500,20}\),  
1000,2,102,44.2938767040396,45,2091.5,421.7976519,71.2339344732021,72,22271.984375,7206.5005709,0.608211783971159,0.6,29796,204,118,95,10,1979,5,2.93550439838905,G1000.0025, \(G_{1000,2.5}\),  
1000,2,451,306.240421509122,307,1009,204.6536909,377.486827140908,378,4701.4375,1400.9069684,0.232648600993595,0.231270358306189,29432,568,54,8,10,1975,4,2.07464583408249,G1000.005, \(G_{1000,5}\),  
1000,2,1367,1112.75608620417,1113,742.9375,152.3545105,1178.93522377057,1179,1881.546875,495.8046354,0.059473175107179,0.059299191374663,21285,799,41,4,9,1329,2,2.48280248134331,G1000.01, \(G_{1000,10}\),  
1000,2,3389,3006.9639862136,3007,683.25,140.6909266,3078.42218408485,3079,1383.421875,374.942909,0.023764234689499,0.023944130362488,15471,1242,25,6,6,1208,2,2.02000776204759,G1000.02, \(G_{1000,20}\),  
500,2,2,0.268496303387567,1,429.359375,74.4340328,1.30949355484287,2,4836.6875,1391.3841535,3.87713811445907,1,15000,0,45,0,10,3136,1,0.010312142302437,U500.05, \(U_{500,5}\),  
500,2,26,7.19052052652705,8,228.125,39.5222584,18.5932309870202,19,1408.28125,393.37937,1.58579763710104,1.375,9921,5079,59,41,10,1770,4,0.007891370063054,U500.10, \(U_{500,10}\),  
500,2,178,55.2543976988495,56,379.75,66.2750358,134.607460122003,135,2040.015625,565.4107938,1.43614021196372,1.41071428571429,10439,4561,60,39,10,2782,4,0.008989963481828,U500.20, \(U_{500,20}\),  
500,2,412,162.799455136723,163,550.9375,97.4653066,338.378649393828,339,3484.4375,1004.6492281,1.07849988877204,1.07975460122699,8739,6261,66,71,10,3326,4,0.006856359327158,U500.40, \(U_{500,40}\),  
1000,2,1,-0.370648806768082,0,3470.1875,725.581516,-0.2627636719341,0,13898.921875,4498.2202233,0.291071043165361,0,30000,0,58,0,10,6792,4,1.94344304155328,U1000.05, \(U_{1000,5}\),  
1000,2,39,7.58691904119982,8,3265.640625,674.9015202,21.4706793587232,22,7291.171875,2284.0963077,1.82996025687494,1.75,25014,4986,63,46,10,3583,4,1.31098518555584,U1000.10, \(U_{1000,10}\),  
1000,2,222,50.5734086572461,51,1037.5625,213.6737431,132.297883177871,133,5928.359375,1840.4606781,1.61595741102801,1.6078431372549,21093,8907,67,72,10,2827,4,1.02976016296414,U1000.20, \(U_{1000,20}\),  
1000,2,737,239.384802540148,240,2724.609375,561.0779492,570.11914703267,571,11695.96875,3685.7005806,1.38160125865573,1.37916666666667,21429,8571,206,103,10,3310,4,1.00908562262322,U1000.40, \(U_{1000,40}\),

==> largeGraphSparse5n_datafile1.tex <==
n,k,UB,DNN_lb,round_DNN_lb,DNN_cputime,DNN_clocktime,cuts_lb,round_cuts_lb,cuts_cputime,cuts_clocktime,imp_lb,imp_lb_round,TotalTriCuts,TotalCliqueCuts,numClustTri,numClustCliq,cut_add_occasions_total,iter,stopflag,sigma,graph,graph_string,
500,4,96,42.6876558538663,43,121.453125,19.9132499,69.67360411377,70,5007.03125,1491.2907212,0.632172175307198,0.627906976744186,24966,34,91,4,10,1419,4,0.018761424620692,G500.005, \(G_{500,2.5}\),
500,4,375,252.420406489872,253,60.609375,10.7848161,296.031131013927,297,3073.3125,867.973167,0.172770201627121,0.173913043478261,23646,23,180,2,10,1063,4,0.016072308262771,G500.01, \(G_{500,5}\), 
500,4,1016,805.858848841064,806,41.046875,6.8117214,833.254051934914,834,279.125,70.8079464,0.033995039122854,0.034739454094293,8737,36,57,2,5,380,3,0.023394473258823,G500.02, \(G_{500,10}\),
500,4,2753,2417.37933963608,2418,33.65625,5.6084872,2433.33202150294,2434,92.734375,27.9326744,0.006599163650195,0.006617038875103,5232,44,19,1,4,254,3,0.019922971794042,G500.04, \(G_{500,20}\),  
1000,4,200,73.5391131443667,74,866.78125,174.1145391,116.220389425989,117,21393.75,7204.3080057,0.580388781651928,0.581081081081081,49998,2,129,1,10,1519,5,0.847423054052297,G1000.0025, \(G_{1000,2.5}\),  
1000,4,767,484.854031979177,485,406,81.8150069,569.686166826029,570,10987.75,3446.472681,0.174964276362861,0.175257731958763,50000,0,230,0,10,1340,4,0.626346186628485,G1000.005, \(G_{1000,5}\),
1000,4,2219,1731.69658444303,1732,261.9375,52.4609123,1773.06805636616,1774,1134.578125,295.2940082,0.023890716361514,0.024249422632795,16558,5,46,1,4,636,2,0.893895621521943,G1000.01, \(G_{1000,10}\),
1000,4,5422,4619.74083994534,4620,223.6875,45.2290173,4639.61108724888,4640,539.4375,132.933149,0.00430116060445,0.004329004329004,8229,12,25,1,3,414,2,0.764350812050851,G1000.02, \(G_{1000,20}\),
500,4,22,1.05156914897908,2,298.125,50.0211797,5.35013268820948,6,5396.046875,1596.1992031,4.08776117424487,2,23854,1146,66,25,10,2966,4,0.014264785281892,U500.05, \(U_{500,5}\),
500,4,115,24.0707782004054,25,268.65625,46.0211691,53.3345003189793,54,3947.46875,1208.5142455,1.21573643672563,1.16,24672,328,94,17,10,1560,4,0.012651533416153,U500.10, \(U_{500,10}\),  
500,4,358,161.122543990459,162,408.828125,68.6722388,303.685626171525,304,5306.984375,1502.7325753,0.884811514579288,0.876543209876543,24228,772,127,11,10,2061,4,0.012350204855651,U500.20, \(U_{500,20}\),  
500,4,1020,548.877957642629,549,560.71875,94.5553227,926.569934392695,927,5675.28125,1644.2687833,0.688116495645429,0.688524590163934,23946,1054,82,8,10,2546,4,0.01046645707278,U500.40, \(U_{500,40}\),  
1000,4,11,0.16844183920266,1,3190.6875,649.013279,2.44609330288518,3,15007.3125,5195.1424953,13.5218866907656,2,50000,0,70,0,10,4565,4,0.622084237819619,U1000.05, \(U_{1000,5}\),  
1000,4,182,22.1144250346585,23,1008.84375,218.2294309,50.8001335637699,51,8727.328125,2929.2376132,1.29714919036575,1.21739130434783,49820,180,107,11,10,2081,4,0.505453381364461,U1000.10, \(U_{1000,10}\),  
1000,4,735,159.511158938809,160,2016.390625,433.6054624,361.072671740729,362,15114.796875,4847.5399016,1.26362013882203,1.2625,49447,553,68,8,10,2832,4,0.472246799785497,U1000.20, \(U_{1000,20}\),  
1000,4,1596,670.640083004918,671,2561.375,534.8845554,1341.68013667791,1342,17488.875,5502.6131224,1.00059640137566,1,49100,900,106,7,10,3147,4,0.429883979375792,U1000.40, \(U_{1000,40}\), 

==> largeGraphSparse5n_datafile2.tex <==
n,k,UB,DNN_lb,round_DNN_lb,DNN_cputime,DNN_clocktime,cuts_lb,round_cuts_lb,cuts_cputime,cuts_clocktime,imp_lb,imp_lb_round,TotalTriCuts,TotalCliqueCuts,numClustTri,numClustCliq,cut_add_occasions_total,iter,stopflag,sigma,graph,graph_string,
500,5,108,48.0187194230034,49,101.828125,17.4713512,77.2031464551006,78,4709.203125,1366.4696294,0.607771872777523,0.591836734693878,24973,27,85,11,10,1416,4,0.02089969834316,G500.005, \(G_{500,2.5}\),
500,5,403,278.160552752331,279,51.046875,8.7709247,318.848720946983,319,2331.265625,625.0907441,0.146275838870942,0.14336917562724,19998,2,234,1,8,924,2,0.021164395432579,G500.01, \(G_{500,5}\),  
500,5,1113,879.394660407565,880,32.796875,5.5605928,898.251491096982,899,222.21875,57.7423299,0.021442967007188,0.021590909090909,6387,0,59,0,4,304,3,0.030899332299748,G500.02, \(G_{500,10}\),  
500,5,2987,2617.06078169391,2618,26.5,4.4731032,2623.49612295622,2624,68.984375,22.9317584,0.002458995720437,0.002291825821238,2868,1,18,1,3,207,3,0.026219845812912,G500.04, \(G_{500,20}\),  
1000,5,228,82.105152438675,83,753.78125,157.9229249,132.558711993473,133,21844.203125,7207.6395598,0.614499310411513,0.602409638554217,50000,0,123,0,10,1514,5,0.57222499452949,G1000.0025, \(G_{1000,2.5}\),  
1000,5,854,531.176113596579,532,331.703125,71.1344118,611.66684398689,612,9673.203125,2758.9802691,0.151533038346379,0.150375939849624,45000,0,262,0,9,1140,2,0.514698724265668,G1000.005, \(G_{1000,5}\),  
1000,5,2449,1880.46382990491,1881,206.015625,40.9094262,1907.65069482967,1908,831.265625,205.347577,0.014457531430496,0.014354066985646,11499,0,43,0,3,510,2,0.757529271654812,G1000.01, \(G_{1000,10}\),  
1000,5,5904,4989.72222565542,4990,171.03125,35.0489147,4996.34731659005,4997,309.53125,66.8661241,0.001327747444651,0.001402805611222,4215,0,31,0,2,285,3,0.651347328508832,G1000.02, \(G_{1000,20}\),  
500,5,21,2.09883985525338,3,203.96875,34.3601209,7.84934885316621,8,4309.703125,1391.0097217,2.7398512485454,1.66666666666667,24772,228,71,7,10,1770,4,0.01910761777319,U500.05, \(U_{500,5}\),  
500,5,98,34.6255438531403,35,282.03125,48.8784312,71.3475010661459,72,4470.28125,1310.7587054,1.06054528323821,1.05714285714286,24744,256,130,5,10,1812,4,0.016730711221404,U500.10, \(U_{500,10}\),  
500,5,439,215.48643151787,216,395.796875,67.6081903,372.230561988345,373,4458.796875,1302.05874,0.727396752391236,0.726851851851852,24638,362,89,9,10,1911,4,0.015829238576651,U500.20, \(U_{500,20}\),  
500,5,1230,770.710382371067,771,500.296875,85.3656381,1164.09274224706,1165,6419.46875,1807.1768759,0.510415285526275,0.511024643320363,24090,910,177,9,10,2499,4,0.011659874830473,U500.40, \(U_{500,40}\),  
1000,5,29,0.284714317141351,1,2565.890625,529.2836963,3.02809747972145,4,15277.71875,5104.2754681,9.63556448486608,3,50000,0,57,0,10,3908,4,0.472145604913791,U1000.05, \(U_{1000,5}\),  
1000,5,220,33.6943972068554,34,847.84375,175.3289423,75.9172935373199,76,9689.453125,3285.8318054,1.25311327195591,1.23529411764706,49879,121,85,5,10,2058,4,0.431918005099387,U1000.10, \(U_{1000,10}\),  
1000,5,716,215.261715172515,216,1994.140625,411.0729014,468.694085573128,469,14944.390625,4581.5154252,1.17732208069376,1.1712962962963,49336,664,81,7,10,2706,4,0.415694089206987,U1000.20, \(U_{1000,20}\),  
1000,5,1836,886.454545399997,887,2427.984375,497.6850373,1608.82308624678,1609,16748.265625,4864.6187702,0.814896313178502,0.813979706877114,49010,990,146,8,10,2625,4,0.308837723006811,U1000.40, \(U_{1000,40}\),

==> largeGraphSparse5n_datafile3.tex <==
n,k,UB,DNN_lb,round_DNN_lb,DNN_cputime,DNN_clocktime,cuts_lb,round_cuts_lb,cuts_cputime,cuts_clocktime,imp_lb,imp_lb_round,TotalTriCuts,TotalCliqueCuts,numClustTri,numClustCliq,cut_add_occasions_total,iter,stopflag,sigma,graph,graph_string,
500,2,49,24.8999946365116,25,266.625,45.8307645,44.3788001371166,45,4609.6875,1425.01329,0.782281513910154,0.8,24549,451,85,59,10,1444,4,0.014777867563098,G500.005, \(G_{500,2.5}\),
500,2,218,155.578188913135,156,133.03125,22.596964,196.610031556718,197,2144.078125,592.328893,0.263737757395367,0.262820512820513,24356,644,98,7,10,1188,4,0.011339431611836,G500.01, \(G_{500,5}\), 
500,2,626,512.133506337669,513,94.234375,15.9009213,553.434944993851,554,567.765625,125.1503322,0.080645843603426,0.079922027290448,13069,713,58,4,8,678,2,0.016211681405011,G500.02, \(G_{500,10}\),
500,2,1744,1565.591086041,1566,86.75,14.7806008,1612.88758266649,1613,192.015625,42.9080801,0.030209993559105,0.030012771392082,9705,1076,18,5,6,520,3,0.013178998854968,G500.04, \(G_{500,20}\),
1000,2,102,44.2938767040396,45,2091.5,421.7976519,73.3326588074606,74,21443.890625,7206.8587673,0.655593600385235,0.644444444444444,44815,185,118,7,9,1731,5,2.63270815171919,G1000.0025, \(G_{1000,2.5}\),
1000,2,451,306.240421509122,307,1009,204.6536909,378.977854701301,379,6977.609375,2183.88006,0.237517414695736,0.234527687296417,49054,946,152,9,10,1822,4,1.85333436577108,G1000.005, \(G_{1000,5}\),
1000,2,1367,1112.75608620417,1113,742.9375,152.3545105,1178.94455268326,1179,1947.53125,523.8239187,0.059481558716854,0.059299191374663,25413,1272,46,5,7,1251,2,2.48296320694699,G1000.01, \(G_{1000,10}\),
1000,2,3389,3006.9639862136,3007,683.25,140.6909266,3078.70867766825,3079,1311.65625,350.83682,0.023859511382107,0.023944130362488,19195,1813,25,7,6,1078,2,2.01714740526152,G1000.02, \(G_{1000,20}\),
500,2,2,0.268496303387567,1,429.359375,74.4340328,1.459128417606,2,8257.21875,2528.18655,4.43444508991913,1,25000,0,98,0,10,3062,1,0.00981228859779,U500.05, \(U_{500,5}\),  
500,2,26,7.19052052652705,8,228.125,39.5222584,22.4796727665861,23,2455.3125,708.106613,2.12629283007465,1.875,17824,7176,67,51,10,1742,4,0.007632283104375,U500.10, \(U_{500,10}\),  
500,2,178,55.2543976988495,56,379.75,66.2750358,152.107251661071,153,3004.84375,838.7393735,1.75285331115351,1.73214285714286,14817,10183,66,50,10,2638,4,0.008116341101737,U500.20, \(U_{500,20}\),  
500,2,412,162.799455136723,163,550.9375,97.4653066,378.901427004252,379,5467.296875,1562.3088117,1.32741213222146,1.32515337423313,17444,7556,120,74,10,3024,4,0.005710119061765,U500.40, \(U_{500,40}\),  
1000,2,1,-0.370648806768082,0,3470.1875,725.581516,-0.162284216340162,0,21411.796875,7200.3132442,0.562161773147958,0,50000,0,81,0,10,6237,5,1.83344306914098,U1000.05, \(U_{1000,5}\),  
1000,2,39,7.58691904119982,8,3265.640625,674.9015202,23.8982739838007,24,8886.578125,3086.5555022,2.14993132970368,2,43836,6164,62,43,10,3357,4,1.29514306884821,U1000.10, \(U_{1000,10}\),  
1000,2,222,50.5734086572461,51,1037.5625,213.6737431,135.032392820123,136,11479,3877.1344094,1.67002751851838,1.66666666666667,42215,7785,95,68,10,3016,4,1.08032041849132,U1000.20, \(U_{1000,20}\),  
1000,2,737,239.384802540148,240,2724.609375,561.0779492,639.201849376332,640,14500.015625,4665.7659204,1.67018558652707,1.66666666666667,40190,9810,197,72,10,3199,4,0.928907459903531,U1000.40, \(U_{1000,40}\),

==> largeGraphSparseSpinglass2pm_datafile1.tex <==
n,k,UB,DNN_lb,round_DNN_lb,DNN_cputime,DNN_clocktime,cuts_lb,round_cuts_lb,cuts_cputime,cuts_clocktime,imp_lb,imp_lb_round,TotalTriCuts,TotalCliqueCuts,numClustTri,numClustCliq,cut_add_occasions_total,iter,stopflag,sigma,graph
324,3,-256,-291.178601529681,-291,79.25,11.4042802,-270.397541918309,-270,3643.0625,1095.0991726,0.072734058816208,0.072164948453608,5274,7686,28,228,8,1797,2,0.008171313664088,spinglass2pm\_18
441,3,-352,-395.508367217053,-395,212.1875,34.6270265,-370.148108347892,-370,4791.34375,1204.8967205,0.06449513924709,0.063291139240506,3280,5540,21,118,4,2786,2,0.026643095479211,spinglass2pm\_21
576,3,-453,-512.168196967489,-512,361.71875,67.5348028,-474.761268817398,-474,6824.671875,1962.9361564,0.074522778246444,0.07421875,3662,7858,23,178,4,2178,2,0.025166115568664,spinglass2pm\_24
729,3,-580,-656.335813442165,-656,579.71875,114.6197084,-607.871903886472,-607,9897.625,3169.0449126,0.075168553096962,0.07469512195122,7289,7291,21,191,4,2587,2,0.021365845025206,spinglass2pm\_27
900,3,-723,-809.707870922529,-809,1103.375,219.8444316,-748.800132442712,-748,20625.359375,6713.4085852,0.076210042088665,0.07540173053152,7922,10078,30,147,4,3442,2,1.85964190051141,spinglass2pm\_30
324,4,-263,-293.618696178475,-293,64.359375,9.6263322,-271.481419431818,-271,1755.3125,297.8498605,0.077034250450885,0.075085324232082,6417,63,51,13,4,1003,2,0.010712137133537,spinglass2pm\_18
400,4,-326,-361.441105561873,-361,91.796875,14.4523586,-333.524483401064,-333,837.171875,164.2482503,0.078688077045527,0.077562326869806,7821,179,50,24,4,487,2,0.011960535007509,spinglass2pm\_20
484,4,-399,-441.131105886212,-441,178.15625,29.4700338,-408.067757238916,-408,1441.421875,408.025362,0.075104896127543,0.074829931972789,16686,254,125,20,7,535,2,0.045520319053496,spinglass2pm\_22
576,4,-465,-516.648211568463,-516,257.65625,47.8307068,-475.335636535165,-475,2510.703125,668.2482574,0.080612321180839,0.079457364341085,16769,511,80,26,6,740,2,0.03720117047107,spinglass2pm\_24
676,4,-551,-611.352804788407,-611,282.78125,55.2733323,-562.777399546412,-562,3054.71875,897.1684478,0.080727207599037,0.080196399345336,19628,652,70,37,6,687,2,0.036634135416251,spinglass2pm\_26
784,4,-635,-709.926903782666,-709,491.890625,97.8833255,-656.1843818751,-656,10223.4375,3102.6320889,0.07596120599928,0.07475317348378,19350,250,49,55,5,1500,2,0.027967391566658,spinglass2pm\_28
1024,4,-823,-922.875353984384,-922,858.609375,170.9051593,-842.642117405745,-842,12901.484375,3978.2176919,0.087634103170289,0.086767895878525,15198,162,38,27,3,1572,2,1.84243002153364,spinglass2pm\_32
400,5,-327,-362.324505631084,-362,91.328125,14.3141306,-333.201448431096,-333,1200.296875,225.3089327,0.080934370089066,0.080110497237569,8000,0,41,0,4,695,2,0.011472741548971,spinglass2pm\_20
625,5,-507,-566.994211555681,-566,338.5625,64.7077875,-515.712370921972,-515,4680.3125,1221.1160643,0.091701485651895,0.090106007067138,12500,0,33,0,4,1150,2,0.043060285896647,spinglass2pm\_25
900,5,-736,-818.707920949541,-818,765.515625,151.5312092,-751.934110989312,-751,7011.875,2110.8321028,0.082700947696968,0.081907090464548,22500,0,57,0,5,1116,2,1.28164037422537,spinglass2pm\_30

==> largeGraphSparseSpinglass3pm_datafile1.tex <==
n,k,UB,DNN_lb,round_DNN_lb,DNN_cputime,DNN_clocktime,cuts_lb,round_cuts_lb,cuts_cputime,cuts_clocktime,imp_lb,imp_lb_round,TotalTriCuts,TotalCliqueCuts,numClustTri,numClustCliq,cut_add_occasions_total,iter,stopflag,sigma,graph
729,3,-769,-902.290043930694,-902,464.875,98.1200456,-821.29763623073,-821,18295.09375,6438.3545525,0.089763162349806,0.08980044345898,20349,12456,44,78,9,2177,2,0.009958700652403,spinglass3pm\_9
512,4,-562,-643.692903205767,-643,169.40625,29.3125109,-590.246516793447,-590,8629.921875,2352.3418632,0.083030877218224,0.082426127527216,17633,287,48,17,7,2355,2,0.019200813095998,spinglass3pm\_8
1000,4,-1058,-1258.4608671532,-1258,1326.765625,265.9521073,-1152.2622856222,-1152,22255.859375,7202.4855742,0.08438767092634,0.084260731319555,24790,210,40,10,5,2523,5,0.845751147512099,spinglass3pm\_10
1000,5,-1068,-1263.77432917812,-1263,1079.484375,207.4967178,-1152.81563486836,-1152,23527.765625,7202.2619191,0.087799452598409,0.087885985748219,30000,0,41,0,6,2482,5,0.633068540455538,spinglass3pm\_10

==> spinglass2pmBisection_datafile1.tex <==
n,m1,UB,DNN_lb,round_DNN_lb,DNN_cputime,DNN_clocktime,cuts_lb,round_cuts_lb,cuts_cputime,cuts_clocktime,imp_lb,imp_lb_round,TotalBQPTriCuts,numClustBQP,cut_add_occasions_total,iter,stopflag,graph,graph_string,
324,195,-222,-245.449421593437,-245,1707.3125,252.0151955,-227.492522413111,-227,27086.84375,7200.074992,0.073159264600224,0.073469387755102,12960,127,8,35081,5,spinglass2pm\_18,spinglass2pm\_18,
400,280,-258,-267.923988831801,-267,4889.78125,735.5972417,-262.569332388747,-262,31207.78125,7200.3941737,0.019985729782544,0.0187265917603,14000,218,7,47002,2,spinglass2pm\_20,spinglass2pm\_20,
441,287,-294,-318.319164273528,-318,4341.46875,667.6976549,-304.395181141394,-304,30236.5625,7200.2525878,0.043742208119677,0.044025157232704,15435,157,7,41725,5,spinglass2pm\_21,spinglass2pm\_21,
484,291,-336,-369.955486084447,-369,5483.625,831.9145873,-347.038390103933,-347,31932.65625,7200.6400448,0.061945549782394,0.059620596205962,24200,146,10,34795,5,spinglass2pm\_22,spinglass2pm\_22,
500,350,173,126.446926310574,127,5250.546875,804.2226209,148.685401834865,149,30331.296875,7200.6297621,0.175872013445946,0.173228346456693,20000,143,10,32734,5,G500.01,\(G_{500,5}\),
500,325,563,462.159519658154,463,3438.828125,518.0066466,489.032608843123,490,15208.46875,3101.6578603,0.058146782749052,0.058315334773218,11361,67,8,22746,2,G500.02,\(G_{500,10}\),
500,300,1682,1496.26372329061,1497,2841.40625,426.1252629,1533.13991563716,1534,12208.15625,2405.5408881,0.024645516544002,0.024716098864396,9646,60,6,21665,2,G500.04,\(G_{500,20}\),
1000,650,387,259.204673099794,260,31575.375,5048.1200272,270.527590050291,271,42869.125,7200.384752,0.043683305609761,0.042307692307692,8000,44,2,26970,5,G1000.005,\(G_{1000,5}\),
1000,600,1304,1047.76028757542,1048,21267.375,3400.2076212,1073.93102439008,1074,40751.265625,7200.4867623,0.024977790363885,0.024809160305344,16000,52,4,22496,5,G1000.01,\(G_{1000,10}\),
1000,700,2844,2502.91563892708,2503,30919.890625,4952.7372983,2513.2697661136,2514,42535.34375,7200.6638274,0.004136826277917,0.004394726328406,12000,70,3,26158,2,G1000.02,\(G_{1000,20}\),
